Identifying Grey-box Thermal Models with Bayesian Neural Networks

Smart thermostats are one of the most prevalent home automation products. They learn occupant preferences and schedules, and utilize an accurate thermal model to reduce the energy use of heating and cooling equipment while maintaining the temperature for maximum comfort. Despite the importance of having an accurate thermal model for the operation of smart thermostats, fast and reliable identification of this model is still an open problem. In this paper, we explore various techniques for establishing a suitable thermal model using time series data generated by smart thermostats. We show that Bayesian neural networks can be used to estimate parameters of a grey-box thermal model if sufficient training data is available, and this model outperforms several black-box models in terms of the temperature prediction accuracy. Leveraging real data from 8,884 homes equipped with smart thermostats, we discuss how the prior knowledge about the model parameters can be utilized to quickly build an accurate thermal model for another home with similar floor area and age in the same climate zone. Moreover, we investigate how to adapt the model originally built for the same home in another season using a small amount of data collected in this season. Our results confirm that maintaining only a small number of pre-trained thermal models will suffice to quickly build accurate thermal models for many other homes, and that 1~day smart thermostat data could significantly improve the accuracy of transferred models in another season.

==> sections/threat.tex <==
\section{Discussion}
% \subsection{RC parameter estimation model}
{\color{red}
One important application of our BNN-$n$R$n$C model is to estimate the $R$ and $C$ values of the building, which can be used for insulation checks and other applications that need the knowledge of the building envelope. The BNN helps estimate the lumped RC parameters based on Equation~(\ref{eq:rc-solution}), but it is non-trivial to extract $R$ and $C$ values from these parameters.

To estimate $R$ and $C$ values, we introduce some errors into the RC model. Equations~(\ref{eq:3r3c}) are the derivative functions of temperature over time. We can estimate the change of temperature by calculating the area between $t$ and $t+\delta$ under the derivative function. We determine the area in Section~\ref{sec:methodology} using definite integral. Alternatively, we can estimate the area by rounding it to a right-angled trapezoid, with height of $\delta$ and two bases of $T'_i(t)$ and $T'_i(t+\delta)$. This allows to identify the exact composition of those lumped RC parameters. For instance, the 2R2C model can be expressed as:
% hard to expand the equation to the form of $R$, $C$, $Q$. This makes the estimation of $R$, and $C$ values nearly impossible. To retrieve the $R$ and $C$ values easily, we introduce some errors into the RC model. Equations~(\ref{eq:3r3c}) are the derivative function of the temperature function over time, and in Equation~(\ref{eq:state}) we find the change of temperature by calculating the area under the derivative function, above the x-axis, and between $t$ and $t+\delta$ using definite integral. To simplify the calculation, we assume the area is a right-angled trapezoid, with height of $\delta$ and two bases of $T'_i(t)$ and $T'_i(t+\delta)$. After this simplification, we can have the exact composition of those lumped RC parameters. For instance, the 2R2C model can be expressed as:
\begin{equation}
\begin{aligned}
    T_{in}^{[t]}=
    &-\frac{2-4C_1R_1}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}T_{in}^{[t-\delta]}\\
    &-\frac{1-2C_1R_1-2C_2R_2-2C_2R_1+4C_1C_2R_1R_2}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}T_{in}^{[t-2\delta]}\\
    &+\frac{R_2Q_{heat}+R_1Q_{heat}-2C_1R_1R_2Q_{heat}}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}k_{heat}^{[t]}\\
    &+\frac{2R_2Q_{heat}+2R_1Q_{heat}-4C_1R_1R_2Q_{heat}}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}k_{heat}^{[t-\delta]}\\
    &+\frac{R_2Q_{heat}+R_1Q_{heat}-2C_1R_1R_2Q_{heat}}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}k_{heat}^{[t-2\delta]}\\
    &-\frac{R_2Q_{cool}+R_1Q_{cool}-2C_1R_1R_2Q_{cool}}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}k_{cool}^{[t]}\\
    &-\frac{2R_2Q_{cool}+2R_1Q_{cool}-4C_1R_1R_2Q_{cool}}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}k_{cool}^{[t-\delta]}\\
    &-\frac{R_2Q_{cool}+R_1Q_{cool}-2C_1R_1R_2Q_{cool}}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}k_{cool}^{[t-2\delta]}\\
    &+\frac{1}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}T_{out}^{[t]}\\
    &+\frac{2}{1-2C_1R_1+2C_2R_2+2C_2R_1-4C_1C_2R_1R_2}T_{out}^{[t-\delta]}\\
    &+\frac{1}{1-2C_1R_1-2C_2R_2-2C_2R_1+4C_1C_2R_1R_2}T_{out}^{[t-2\delta]}\\
\end{aligned}
\label{eq:final}
\end{equation}

The error depends on the temperature fluctuation rate. If the rate varies a lot during $t$ and $t+\delta$, then the error is significant. Since our $\delta$ is 5 minutes, and we are considering residence building only, the rate is nearly stable within the 5-minute interval in the real-world scenario. 
This is because the residence building usually does not have a powerful HVAC system.

Despite the fact that now we have a system of equations~(\ref{eq:final}) since we know the value of each parameter, this system of equations is under-determined. We have to at least know one value to make the system of equations solvable. Although the value of $Q_{heat}$ and $Q_{cool}$ is not available in our dataset, but it is usually easy to retrieve from the HVAC system, which makes $R$ and $C$ values solvable.
}
